Checking Information Flow in Cloud-based IoT Access Control Policies (Extended Version)

Many cloud providers for IoT technologies offer access control mechanisms whose proper configuration is critical for security. However, verifying permissions in isolation is insufficient in a setting where devices have different levels of trust or are compartmentalised in various subsystems. This work analyses IoT access control policies to identify potential security vulnerabilities from unwanted information flow between devices. To this end, we formally model AWS IoT Core's components and define an information flow graph to capture the communication among devices permitted by the access control policies. We build a finite representation of the graph by leveraging an SMT solver, thus enabling the verification of information flow between devices. We implement our approach in a tool called IOT:POKER, and assess it on a realistic scenario and several real-world policies.

==> IoTmacros.tex <==
\ProvidesPackage{IoTmacros}[2024/10/22 v1.2 IoT macros]

\newcommand{\code}[1]{\text{\small$\mathtt{#1}$}}
\newcommand{\codea}[1]{\mathtt{#1}}
\newcommand{\mathExpa}[1]{\operatorname{\codea{#1}}}
\newcommand{\mathExp}[1]{\operatorname{\code{#1}}}
\newcommand{\codeExp}[1]{\texttt{\textup{#1}}\xspace}
\newcommand{\Set}[1]{\mathbb{#1}}
\newcommand{\SetOfSets}[1]{\mathscr{#1}}
\newcommand{\Ast}{\textnormal{*}}

\newcommand{\readOP}{\codeExp{read}}
\newcommand{\writeOP}{\codeExp{write}}
\newcommand{\executeOP}{\codeExp{execute}}
\newcommand{\deleteOP}{\codeExp{delete}}



\newcommand{\rExp}{\mathExp{Re}}
\newcommand{\tExp}{\mathExp{Tre}}
\newcommand{\tfExp}{\mathExp{TFre}}
\newcommand{\cExp}{\mathExp{Cre}}
\newcommand{\re}{\rExp}
\newcommand{\RE}{\mathcal{R}} %
\newcommand{\RExp}{\SetOfSets{R}} %
\newcommand{\lang}[1]{\mathcal{L}(#1)}
\newcommand{\AWS}{\mathtt{aws}}
\newcommand{\mqtt}{\mathtt{mqtt}}

\newcommand{\allow}{\mathExp{Allow}}
\newcommand{\deny}{\mathExp{Deny}}
\newcommand{\allowa}{\mathExpa{Allow}}
\newcommand{\denya}{\mathExpa{Deny}}
\newcommand{\defDeny}{\mathsf{Default\,Deny}}
\newcommand{\iotConn}{\mathExp{Con}}
\newcommand{\iotPub}{\mathExp{Pub}}
\newcommand{\iotRec}{\mathExp{Rec}}
\newcommand{\iotSub}{\mathExp{Sub}}
\newcommand{\effect}{\varepsilon}
\newcommand{\action}{\alpha}
\newcommand{\actions}{\Set{A}}

\newcommand{\certs}{\Set{C}}
\newcommand{\pol}{P}
\newcommand{\pols}{\Set{P}}
\newcommand{\gpol}{\pol^r}
\newcommand{\iotvar}[1]{\underline{\$#1}}
\newcommand{\cidVAR}{\code{\iotvar{clientId}}}
\newcommand{\cidVARa}{\codea{\iotvar{clientId}}}
\newcommand{\tname}{\mathExp{thingName}}
\newcommand{\tnameVAR}{\code{\iotvar{thingName}}}
\newcommand{\thing}{T}
\newcommand{\things}{\Set{T}}
\newcommand{\topics}{\Set{T}}
\newcommand{\topicfs}{\Set{TF}}
\newcommand{\cids}{\Set{I}}

\newcommand{\msg}{m}
\newcommand{\bstate}{\sigma}
\newcommand{\conns}{\Set{L}}
\newcommand{\inpols}{p}
\newcommand{\subs}{\varsigma}

\newcommand{\redef}[3]{#1 \triangleleft [#2 \mapsto #3]}

\newcommand{\cid}{\operatorname{\mathit{id}}}
\newcommand{\tf}{\operatorname{\mathit{tf}}}
\newcommand{\res}{\rho}
\newcommand{\req}[1][]{(c, \cid, \action_#1, \res)}
\newcommand{\reqs}{\Set{R}}

\newcommand{\Allow}{\mathtt{A}}
\newcommand{\Deny}{\mathtt{D}}
\newcommand{\DefDeny}{\mathtt{d}}
\newcommand{\decs}{\Set{D}}

\newcommand{\polState}{(\varepsilon, \alpha, \RE)}
\newcommand{\iotConf}{(\certs, \pols, \varphi)}
\newcommand{\reqEval}[1]{\psi_{#1}}
\newcommand{\REallow}{eval_a}
\newcommand{\Fin}{\mathcal{I}}
\newcommand{\Fout}{\mathcal{O}}
\newcommand{\Sin}{\topics^I}
\newcommand{\Sout}{\topics^O}


\newcommand{\clientID}{\$\textit{clientid}}
\newcommand{\mqttConn}{\codeExp{Con}}
\newcommand{\mqttCAck}{\codeExp{CONNACK}}
\newcommand{\mqttPub}{\codeExp{Pub}}
\newcommand{\mqttSub}{\codeExp{Sub}}
\newcommand{\mqttDis}{\codeExp{Disc}}
\newcommand{\mqttUns}{\codeExp{UnSub}}

\newcommand{\receivers}{Rec}
\newcommand{\con}{\ell}
\newcommand{\Con}{\Set{LLL}}
\newcommand{\Dev}{\Set{D}}
\newcommand{\dev}{d}
\newcommand{\devof}{\mathit{dev}}
\newcommand{\com}{\mathit{tr}}
\newcommand{\Com}{\mathit{Tr}}

\newcommand{\SecLab}{\Set{S}}

